RAD-Sim: Rapid Architecture Exploration for Novel Reconfigurable Acceleration Devices

With the continued growth in field-programmable gate array (FPGA) capacity and their incorporation into new environments such as datacenters, we have witnessed the introduction of a new class of reconfigurable acceleration devices (RADs) that go beyond conventional FPGA architectures. These devices combine a reconfigurable fabric with coarse-grained domain-specialized accelerator blocks all connected via a high-performance packet-switched network-on-chip (NoC) for efficient system-wide communication. However, we lack the tools necessary to efficiently explore the huge design space for RADs, study the complex interactions between their different components and evaluate various combinations of design choices. In this work, we develop RAD-Sim, a cycle-level architecture simulator that allows rapid application-driven exploration of the design space of novel RADs. To showcase the capabilities of RADSim, we map and simulate a state-of-the-art deep learning (DL) inference overlay on a RAD instance incorporating an FPGA fabric and a complex of hard matrix-vector multiplication engines, communicating over a system-wide NoC. Through this example, we show how RAD-Sim can help architects quantify the effect of changing specific architecture parameters on end-to-end application performance.

==> 05_npu_rad.tex <==
\section{NPU on RADs}
\label{sec:npu_rad}

Use of LI bandwidth-driven design (as illustrated for the NPU in the previous section) and a system-level NoC completely decouples the application compute from its inter-module communication.
This raises the interconnect abstraction level and enables the exploration of complex RADs that span multiple dice and incorporate hard accelerator blocks.
In this case, the conventional FPGA CAD tools do not need to optimize the timing and routability of signals crossing the boundaries between dice through interposers or trying to reach the programmable routing interfaces of a hard accelerator block.
If each application module meets timing separately and can be connected to a NoC adapter, the evaluation of end-to-end application performance on a given RAD instance is raised to the cycle-level simulation of soft/hard modules and NoC latency; this is exactly what is captured by RAD-Sim.

\subsection{Experimental Setup \& Methodology}
\label{sec:setup}

We map the re-designed LI AXI-S multi-threaded NPU to three example RADs and evaluate their performance using RAD-Sim.
The first device (RAD1), illustrated in Fig. \ref{fig:rad-scenarios}a, consists of two identical FPGA fabrics using 2.5D chip integration \cite{nasiri2015multiple} where the NoC links are the only wires crossing from one fabric to another through a passive interposer.
The second one (RAD2) in Fig. \ref{fig:rad-scenarios}b is a monolithic device with an FPGA fabric and a separate complex of hard accelerator blocks.
In this case, the accelerator blocks can only be accessed from the fabric using the NoC.
Finally, the third device (RAD3) is an FPGA fabric 3D-stacked on top of a base die of accelerator blocks similar to that shown in Fig. \ref{fig:rad-instance}.
We define the term \textit{FPGA sector} as a region of FPGA resources with a NoC router/adapter at its center.
For example, an FPGA with 8$\times$5 sectors has a total of 40 NoC routers/adapters throughout its fabric regardless of the NoC topology used (i.e. it does not have to be a regular 8$\times$5 mesh topology).
Equivalently, we define an \textit{ASIC sector} as an area of silicon that has the same footprint of an FPGA sector and includes a hard accelerator block (possibly with other hardened components) and a NoC router.
Table \ref{tab:rad-specs} summarizes the specifications of the three example RADs we use in our study. 

\begin{figure}[t!]
    \centering
    \includegraphics[width=1\linewidth]{Figures/rad-examples-npu-horizontal.pdf}
    \caption{RADs used in our study: (a) 2.5D integration of 2 FPGA fabrics with the NoC links crossing through a passive interposer, and (b) monolithic FPGA fabric and coarse-grained hard accelerators.}
    \label{fig:rad-scenarios}
    \vspace{-0.2cm}
\end{figure}

\begin{table}[t!]
    \centering
    \caption{Specifications of example RADs used in our study.}
    \vspace{-0.2cm}
    \begin{tabular}{C{1cm} C{1.2cm} C{1.2cm} C{1.5cm} C{1.5cm}} 
    \hline\\ [-1.8ex]
    \textbf{} & \textbf{FPGA Sectors} & \textbf{ASIC Sectors} & \textbf{Integration Tech.} & \textbf{NPU Config.}\\ [0.25ex] 
    \hline\\ [-1.8ex]
    \textbf{RAD1} & 8$\times$5 ($\times$2) & -- & 2.5D passive & 1 $\times$ 4-thread \\
    \textbf{RAD2} & 8$\times$5 & 2$\times$5 & Monolithic &  1 $\times$ 4-thread\\
    \textbf{RAD3} & 8$\times$5 & 8$\times$5 & 3D active &  4 $\times$ 1-thread\\ [0.25ex]
    \hline
    \end{tabular}
    \label{tab:rad-specs}
    \vspace{-0.3cm}
\end{table}

For all three example RADs, we begin with an FPGA fabric with the same resources as an Intel Stratix 10 NX 2100 device ($702$k ALMs, $6,847$ M20K BRAMs, $3,960$ TBs).
For RAD3, we assume that the FPGA fabric and the base die are implemented in the same process technology for simplicity. 
We remove resources to make room for any NoC routers added. 
%Note that RAD2 divides its fabric resources into 50 sectors instead of the 40 sectors of RAD1 and RAD3 to better match the ASIC sector count, but each sector is smaller.
We implement matrix-vector multiplication units that resemble the MVU slices of the NPU described in Sec. \ref{sec:bw-npu} as the hard accelerator blocks in RAD2 and RAD3.
These blocks are realistic candidates for hardening since they implement common functionality across almost all AI workloads, while the rest of the NPU blocks could be specialized for different workloads to increase efficiency \cite{boutros2021specializing} and thus benefit from the FPGA's reconfigurability.
For RAD1, we use one FPGA for implementing the NPU's MVU slices (FPGA1) and the other FPGA to instantiate vector EW slices to support 4 interleaved thread executions (FPGA2).
For RAD2 and RAD3, we first stamp out enough single thread NPU copies to utilize all the available hard accelerator blocks, and then use any remaining FPGA resources to add support for as many interleaved thread executions as possible.
Table \ref{tab:rad-specs} lists the NPU configurations used.

\begin{table}[t!]
    \centering
    \caption{Resource utilization for the NPU portions implemented on the RAD FPGAs (TBs: tensor blocks, M20K: 20Kb BRAMs).}
    \vspace{-0.2cm}
    \begin{tabular}{C{2cm} C{2.2cm} C{1.5cm} C{1.5cm}} 
    \hline\\ [-1.8ex]
     & \textbf{ALMs} & \textbf{M20Ks} & \textbf{TBs} \\ [0.25ex] 
    \hline\\ [-1.8ex]
    \textbf{RAD1 - FPGA1}    & 83,585 (12\%) & 5,260 (77\%) & 2,800 (71\%)\\ 
    \textbf{RAD1 - FPGA2}    & 494,216 (70\%) & 5,644 (82\%) & 3,200 (81\%)\\ 
    %RAD2 & \hl{550,0930 (78\%)} & \hl{2,632 (90\%)} & \hl{3,200 (81\%)}\\ 
    \textbf{RAD2 \& RAD3} & 550,0930 (78\%) & 2,632 (90\%) & 3,200 (81\%)\\ [0.25ex]
    \hline
    \end{tabular}
    \label{tab:fpga-resources}
    \vspace{-0.5cm}
\end{table}

\begin{figure*}[t!]
    \centering
    \includegraphics[width=1\linewidth]{Figures/results-combo.pdf}
    \vspace{-0.2cm}
    \caption{(a) Quartus chip planner view of the FPGA fabric of RAD3 with different colors showing the 4 sets of NPU vector EW slices and the small boxes representing reserved logic lock regions for the fabric NoC adapters, (b) Relative performance comparison of the baseline NPU on Stratix 10 NX and the re-designed NPU on the 3 RADs we study, (c) Performance of RAD2 and RAD3 on bigger workloads, (d) Effect of changing NoC VC buffer size on NPU performance.}
    \label{fig:combo}
    \vspace{-0.5cm}
\end{figure*}

We estimate performance by using RAD-Sim to map the NPU to the three example RADs.
We set an FPGA fabric operating frequency of 300 MHz (matching the NPU operating frequency in \cite{boutros2020beyond}) and conservatively assume that the hard accelerator blocks run at 600 MHz.
We scale the operating frequency of the 28nm NoC routers from \cite{abdelfattah2015take} to 1.5 GHz in 14nm process technology, and we assume that the NoC adapters operate at 4$\times$ the fabric speed, similarly to \cite{abdelfattah2015take}.
In all experiments, we use a mesh NoC topology (dimensions specified in Table \ref{tab:rad-specs} for each case) with 3 VCs and dimension order packet routing.
The depths of the NoC adapters' injection/ejection FIFOs and ouptut buffers (see Fig. \ref{fig:noc-adapters}) are set to 16 and 2, respectively.
We also manually assign NPU modules to specific routers in a reasonable (but possibly sub-optimal) placement.

\subsection{FPGA and ASIC Area Results}

%\begin{figure}[t!]
%    \centering
%    \includegraphics[width=0.6\linewidth]{Figures/floorplan.pdf}
%    \caption{Quartus chip planner view of the FPGA fabric of RAD3. Different colors show the 4 instantiations of NPU vector elementwise modules working with hard MVUs on the base die. The small boxes are reserved logic lock regions for the fabric NoC adapters.}
%    \label{fig:floorplan}
%    \vspace{-0.4cm}
%\end{figure}

To determine FPGA resource utilization, we synthesize, place and route the parts of the NPU to be implemented on the FPGA fabrics using Intel Quartus Prime Pro 21.2 on a Stratix 10 NX 2100 device.
We use reserved logic lock regions at the appropriate locations for NoC routers/adapters, mark them as empty design partitions, and connect the NPU modules to them based on our manual module assignment to different routers. 
We conservatively size each logic lock region as a grid of 10$\times$10 logic array blocks (LABs) compared to the 3$\times$3 LAB region used in \cite{abdelfattah2012design}, as we are using 128-bit wide links vs. the 32-bit wide links of \cite{abdelfattah2012design}.
Table \ref{tab:fpga-resources} shows the FPGA resource utilization of the NPU portions implemented on the FPGA fabrics of each of the three RADs and Fig. \ref{fig:combo}a shows the Quartus chip planner view of the FPGA portion implementation of the RAD3 instance.

We also verify that the matrix-vector multiplication units we chose to implement as hard accelerator blocks fit in the available ASIC sector area footprint.
Since the silicon area footprint of Stratix 10 FPGA resources are proprietary information, we estimate the relative area as follows.
First, we implement the matrix-vector multiplication unit on the Stratix 10 NX programmable fabric and convert its resource utilization results into equivalent ALMs \cite{wong2011comparing} to get an area footprint breakdown of different components of the circuit.
This matrix-vector multiplication unit utilizes the equivalent of 2.8 FPGA sectors with 68\%, 21\% and 11\% of its area dedicated to BRAMs, ALMs and TBs, respectively.
\cite{boutros2018you} and \cite{boutros2018embracing} show that ALMs, BRAMs, and DSPs/TBs have 26$\times$, 3$\times$, and 1.35$\times$ smaller area footprint when implemented in an ASIC without any reconfigurability or interfaces to the programmable routing.
Therefore, we use a weighted average of these FPGA-to-ASIC area scaling ratios based on our circuit composition to get an approximate ASIC area footprint.
The hard matrix-vector unit consumes less than 55\% and 40\% of the available ASIC sector area for the 4-thread (RAD2) and 1-thread (RAD3) variations respectively, leaving more than enough area for the NoC routers, adapters, links, and any additional hardened functionality.
In the future, the RAD-Gen component of our flow, described in Sec. \ref{sec:flow-overview}, will automate any manual steps needed to obtain the FPGA results and will push the RTL implementation of the hard accelerator blocks through the ASIC design flow to obtain exact area and timing results.

\subsection{Performance Results}
\label{sec:perf-results}

%\begin{figure}[t!]
%    \centering
%    \includegraphics[width=0.9\linewidth]{Figures/npu_rad_relative.pdf}
%    \caption{(a) Relative performance comparison of the baseline NPU on Stratix 10 NX and the re-designed NPU on the 3 RADs we study, and (b) Performance of RAD2 and RAD3 on bigger workloads.}
%    \label{fig:npu-rad-perf}
%    \vspace{-0.5cm}
%\end{figure}

Fig. \ref{fig:combo}b shows the relative performance comparison between the baseline latency-sensitive NPU on Stratix 10 NX from \cite{boutros2020beyond} and the re-designed NPU mapped to the three RAD instances we use in our study.
Although RAD1 uses two FPGA fabrics, it does not benefit from any increase in the MVU compute resources compared to the baseline NPU. 
It only uses the resources of the second FPGA to add support for 4 interleaved thread executions.
With the overhead of LI re-design and higher-latency NoC communication, RAD1 can achieve only 12\% better performance on average compared to the baseline NPU.
In comparison, the single-die RAD2 achieves 1.2$\times$ (1.32$\times$) the performance of RAD1 (the baseline NPU) by exploiting the hardened MVU coarse-grained accelerator blocks and interleaving four thread executions.
Finally, the base die of RAD3 can implement the MVU slices of 4 NPU instances and frees the FPGA resources to implement the rest of their vector EW, LD and instruction dispatch units.
This results in a significant 2.6$\times$ increase in average performance compared to the baseline NPU on a same form-factor FPGA without 3D stacking.
In addition, since the hard matrix-vector multiplication units in RAD2 and RAD3 are designed to have bigger RFs, they can both run a new set of bigger workloads (shown in Fig. \ref{fig:combo}c) that can not fit in the on-chip memory of the baseline NPU.
These results show that RAD3 can achieve up to 145 TOPS on the LSTM-1536 workload.

Besides its ability to model different RAD architectures, RAD-Sim also enables us to study the effect of different architecture parameters on the performance of application designs.
Fig. \ref{fig:combo}d shows the impact of VC buffer size in the NoC routers of RAD2. 
VC buffer depths less than 8 flits can throttle performance given the NPU traffic patterns over the NoC, while increases beyond 8 flits yield little additional performance.

%\begin{figure}[t!]
%    \centering
%    \includegraphics[width=0.8\linewidth]{Figures/vc.pdf}
%    \caption{Effect of changing NoC VC buffer size on NPU performance.}
%    \label{fig:npu-vc}
%    \vspace{-0.6cm}
%\end{figure}
